Towards Measuring Fairness in Grid Layout in Recommender Systems

There has been significant research in the last five years on ensuring the providers of items in a recommender system are treated fairly, particularly in terms of the exposure the system provides to their work through its results. However, the metrics developed to date have all been designed and tested for linear ranked lists. It is unknown whether and how existing fair ranking metrics for linear layouts can be applied to grid-based displays. Moreover, depending on the device (phone, tab, or laptop) users use to interact with systems, column size is adjusted using column reduction approaches in a grid-view. The visibility or exposure of recommended items in grid layouts varies based on column sizes and column reduction approaches as well. In this paper, we extend existing fair ranking concepts and metrics to study provider-side group fairness in grid layouts, present an analysis of the behavior of these grid adaptations of fair ranking metrics, and study how their behavior changes across different grid ranking layout designs and geometries. We examine how fairness scores change with different ranking layouts to yield insights into (1) the consistency of fair ranking measurements across layouts; (2) whether rankings optimized for fairness in a linear ranking remain fair when the results are displayed in a grid; and (3) the impact of column reduction approaches to support different device geometries on fairness measurement. This work highlights the need to use layout-specific user attention models when measuring fairness of rankings, and provide practitioners with a first set of insights on what to expect when translating existing fair ranking metrics to the grid layouts in wide use today.

==> tables.tex <==
\begin{table}[tb]
\centering
 %\footnotesize
 \caption{Summary of notation.}
 \begin{tabular}{cl}

 \toprule
  $\doc \in \allitems$ & document or item \\
  $\user \in \allusers$ & request (query or user) \\
  $\ranking$ & ranked results of $N$ documents from $\allitems$ \\
  $\ranking^{-1}(i)$ & the document in position $i$ of linear (1-column) layout \\
  $\rankingPosition$ & rank of document $d$ in linear layout \\
  $\itemrow$ & row number of document $d$ in grid layout \\
  $\iteminrow{k}$ & items in $k$th row in grid layout \\
  %$\ranking_{\le k}$ & prefix of $\ranking$ of length $k$ \\
  $\relevance$ & relevance of $d$ to $q$ \\
  $\group$ & number of groups \\
  $\alignmentvec$ & group alignment vector \\
  $\alignmentmat$ & group alignment matrix for documents in $\ranking$ \\
  $\Protected$ & set of documents in protected group in $L$ \\
  $\nonProtected$ & set of documents non-protected group in $L$ \\
  $\populationEstimator$ & target group distribution \\
  %$\probabiltyDist(\ranking)$ & probability distribution of groups in $\ranking$ \\
  $\attentionmat$ & attention vector for documents in $\ranking$ \\
  $\attentionvec$ & position weight of $\doc$ in $\ranking$ \\
  $\groupexposure$ & the exposure of groups in $\ranking$ ($\alignmentmat^T \attentionmat$) \\

\bottomrule
 \end{tabular}
 \label{tab:notation}
\end{table}
